Adversarial Manipulation of Deep Representations

We show that the representation of an image in a deep neural network (DNN) can be manipulated to mimic those of other natural images, with only minor, imperceptible perturbations to the original image. Previous methods for generating adversarial images focused on image perturbations designed to produce erroneous class labels, while we concentrate on the internal layers of DNN representations. In this way our new class of adversarial images differs qualitatively from others. While the adversary is perceptually similar to one image, its internal representation appears remarkably similar to a different image, one from a different class, bearing little if any apparent similarity to the input; they appear generic and consistent with the space of natural images. This phenomenon raises questions about DNN representations, as well as the properties of natural images themselves.

==> discussion.tex <==
\section{discussion}


==> exp_closeness_sara.tex <==
%\subsection{Distance to guide and origin}

\iffalse
\begin{subfigure}[t]{.19\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_intra_all.png}

\caption{$\frac{d(g_i,\adv_{ij}^{F7})}{avg_i}$.}
\label{fig:Guide_Intra}
\end{subfigure}
\fi


\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_init_all_p5.png}
\caption{\tiny{$\left. d(\adv,\guide) \middle/ ~d(\source,\guide) \right.$, on $P5$}}
\label{fig:Guide_Init_p5}
\end{subfigure}
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_init_all.png}
\caption{\tiny{$\left. d(\adv, \guide) \middle/ ~d(\source,\guide) \right.$, on ${\text{FC}7}$}}
\label{fig:Guide_Init}
\end{subfigure}
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_nneigh_all.png}
\caption{\tiny{$\left. {d(\adv,\guide)} \middle/ {~\overline{d_1}(\guide)} \right.$, on ${\text{FC}7}$}}
\label{fig:guide_nneigh}
\end{subfigure}
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/seed_intra_all.png}
\caption{\tiny{
$\left. {d(\source,\adv)} \middle/ {~ \overline{d}(\source)} \right.$, on ${\text{FC}7}$}}
\label{fig:Source_Intra}
\end{subfigure}
\caption{Histogram of the distance between adversarial representations 
    ($\adv$) and their (source:
    $\source$, guide:  $\guide$) pairs, on different layers. The layer where 
    the optimization is performed on is also where distances of representations 
    are computed. Distance between $x$ and $y$ is denoted by $d(x,y)$, while
    $\overline{d}(\source)$ denotes the average pairwise distances of points in 
the class of $\source$ and  $\overline{d_1}(\guide)$ is the average distance to 
the top one nearest neighbor in the class of $\guide$. All distances are
Euclidean, and the histograms aggregate over different choices of sources and guides.}
\label{fig:H_Dist}
\end{figure*}

% \subsubsection{Guide and adversarial distance analysis}
\comment{
\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_init_all_p5.png}
\caption{{\large $~\frac{d(\adv^{P5},\guide)}{d(\source,\guide)}$}}
\label{fig:Guide_Init_p5}
\end{subfigure}
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_init_all.png}
\caption{{\large $~\frac{d(\adv^{\text{FC}7}, \guide)} {d( \source,\guide)}$}}
\label{fig:Guide_Init}
\end{subfigure}
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/guide_nneigh_all.png}
\caption{{\large $~\frac{d(\adv^{\text{FC}7},\guide)} {\text{avg}_{\guide}}$}}
\label{fig:guide_nneigh}
\end{subfigure}
\begin{subfigure}[t]{.245\linewidth}
\includegraphics[width=\linewidth]{./imgs/seed_intra_all.png}
\caption{{\large $~\frac{d(\source,\adv^{\text{FC}7})}{\text{avg}_{\source}}$}}
\label{fig:Source_Intra}
\end{subfigure}
\caption{Histogram of the distance between adversarial representations 
    ($\adv^{L}, L \in \{\text{FC}7, \text{Pool}5\} $) and their (source: 
    $\source$, guide: $\guide$) pairs, $L$ indicates the optimization layer.  
    Distance between $x$ and $y$ is denoted by $d(x,y)$, $\text{avg}_{\source}$ 
    is the average of pairwise distances in the class of image of $\source$ and 
    $\text{avg}_{\guide}$ is the average of distance to the nearest neighbor in 
the class of image of $\guide$.  All distance measurements are Euclidian and 
are calculated on the layer $L$ representations of Caffenet.}
\label{fig:H_Dist}
\end{figure*}
}
% In addition to the qualitative similarity between the internal representations
% for the guide and the adversarial images, shown in Fig.~\ref{fig:adv_invert},
% it is also useful to examine quantitative measures of closeness. We report the
% ratio of adversarial's distance and the source's distance to guide to measure
% the magnitude of enlargment of $\delta$ perturbation of the source for both
% adversarials optimized for FC$7$ and Pool$5$. Also, we examine whether the
% adversarials distance to source and guide are typical of their classes to show
% the relative position of the adversarials in the representational space of
% FC$7$. Finally, the position of the adversarial in the eye of other images from
% the same class is compared to its guide to verify guide and adversarial
% representation are truly measured as identical.



First, we examine distances between internal representations of 
source, guide and adversarial images for a large collection of
source-guide pairs.  We used 20 source images, with five drawn at 
random from each of the ILSVRC training, testing and validation sets, 
and five more selected manually from Wikipedia and the ILSVRC 
validation set to provide greater diversity.
For experiments on layer FC7 the guide set comprised three images from each of 
1000 classes, drawn at random from ILSVRC training and 30 images from each of 
     validation and testing sets. To simplify the reporting of classification 
     behaviour,
we only use guides from training set whose labels are correctly predicted by 
Caffenet.  For other layers (e.g., P5), for computational expedience, we draw 
guide images from just 100 classes. In both cases, we consider all possible 
source-guide combinations from the respective source and guide sets
of images.
To simplify the exposition in what follows, we use $\source$, $\guide$ and 
$\adv$  to denote DNN representations of source, guide and adversarial images, 
whenever there is no confusion about the layer of the representations.

\comment{Based on adversarial images based on all source-guide pairs, }
    Fig.~\ref{fig:H_Dist}\subref{fig:Guide_Init_p5} shows the histogram of the 
    Euclidean distance between the P5 representation of the adervarial $\adv$ 
    and guide $\guide$, divided by the distance between the source $\source$ 
    and guide $\guide$ P5 encodings.
With a ratio less than 1, it is clear that at layer P5, $\adv$ is on
average much close to $\guide$ than $\source$.
If we relax the bound on the maximum deviation from the 
source image, the adversarial representation is even closer to the guide.  
Fig.~\ref{fig:H_Dist}\subref{fig:Guide_Init} shows a similar plot,
but for layer FC7.  With $\delta = 10$ the adversarial FC7 representation 
is 80\% closer to the guide than the source, but as $\delta$ decreases
the constraint becomes stronger and the adversarial FC7 representation
is drawn closer to the source.

% The distance between internal FC$7$ representations of source and guide pairs
% is $110.24$, while the average FC$7$ distances between adversarial with
% $\delta=10$ and guide images is just $13.82$.  between internal FC$7$
% representations of source and guide pairs is $110.24$, while the average
% FC$7$ distances between adversarial with $\delta=10$ and guide images 
Fig.~\ref{fig:H_Dist}\subref{fig:guide_nneigh} compares FC$7$ distances
between $\adv$ and $\guide$ with the average distance between each image from 
the same class and its nearest neighbor (NN) FC7 representation among all 
ILSVRC images of the same label class.
With $\delta=10$, the distance between adversarial and guide FC7 encodings 
is 78\% smaller than the average distance between NNs within the same class.
Finally, Fig.~\ref{fig:H_Dist}\subref{fig:Source_Intra} shows that 
the distance between adversarial and source FC7 encodings is relatively
large compared to typical pairwise distances between FC7 representations
within the same class as the source.  Only $8\%$ of adversarial images  
(at $\delta=10$) are closer to their source than average pairwise distances 
between FC7 representations from the source class.







==> exp_general.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{{{
\subsection{Generating Adversarial Images for Other Networks and Other
Datasets}

We show that we can generate our adversarial images on other networks trained
on ImageNet dataset and Places205 dataset. We repeat the experiments described
in Section~\ref{RankAnalysis} on other networks to show that the generated
adversarial images look like inliers in the guide class for various CNN
networks. For networks trained on Flickr style dataset we show that it is
possible to find adversarials on the last layer before classification but for
layers below, sometimes the optimization quickly ends up in local minima.

The models we analyse are the Caffe Reference Net (Caffenet), AlexNet,
GoogleNet, VGG CNN Slow, AlexNet trained on Places205 dataset to classify 205
classes of scenes, a hybrid model of AlexNet trained to classify 205 scene
classes and 977 classes from ImageNet, and AlexNet finetuned for classification
on Flickr Style dataset. The Places205 dataset has $2.5$ million images of
scenes categorized into 205 classes. The Flickr Style has $80,000$ images from
Flickr, categorized into 20 classes of photo styles.

Table~\ref{tb:generalize_tb1} shows that not only our adversarials almost
always have the label of the guide, but also they are almost always so close to
the guide that the first nearest neighbor of them in the class of the guide is
the guide itself. For all networks, except for FC$7$ on Flickr, the difference
in rank, $\rankdiff{3}$, is better than $-7$ which means that for half of the
adversarials, we are more similar to the guide compared to $93\%$ of other
images in that class.

On the finetuned model on Flickr Style, we observe that we can quickly generate
adversarials that we can optimize the FC$8$, the unnormalized class scores, to
be the same as the guide with $\rankdiff{3}$ being $0.00$. However, when doing
the optimization on FC$7$, for $55$ examples on train-train split and $59$
examples on train-test split, the optimization quickly converges to local
minima. The interesting observation is that, almost always, the local minima
has $\rank{3}=0$. This means that the optimization has converged to the most
dense regions of a class.

We also show that our adversarials generated on one network generalize
partially to other networks. Table~\ref{tb:generalize_tb2} shows the results of
this analysis. We have used the same set of adversarials as in
Table~\ref{tb:generalize_tb2} and evaluated how often an adversarial is
misclassified by the target network and how often we have been successful in
changing the label to the target label. The adversarials are misclassified by
another net in $49.00\pm8.91$ times on train-train splits and $58.83\pm7.32$
times on train-test splits but they are almost never classified to the class of
the guide.

\begin{table*}[ht] \resizebox{\linewidth}{!}{\centering
        \begin{tabular}{|c|c|c|c|c|c|} \hline Model & Layer & Split sets
        & Out $\class{\source}$& In $\class{\guide}$
        & $\guide=\neigh{1}{\adv}$\\
        \hline
%
CaffeNet&       FC$7$&  train-train&    $100$&  $95$&   $95$\\
AlexNet&        FC$7$&  train-train&    $100$&  $97$&   $96$\\
GoogleNet&      pool5/7x7\_s1&  train-train&    $100$&  $100$&  $100$\\
VGG CNN S&      FC$7$&  train-train&    $100$&  $99$&   $99$\\
Places205 AlexNet&      FC$7$&  train-train&    $100$&  $100$&  $98$\\
Places205 Hybrid&       FC$7$&  train-train&    $100$&  $99$&   $99$\\
Flickr Style&   FC$8$ Flickr&   train-train&    $100$&  $100$&  $95$\\
Flickr Style&   FC$7$&  train-train&    $98$&   $45$&   $32$\\
\hline
CaffeNet&       FC$7$&  train-test&     $100$&  $97$&   $96$\\
AlexNet&        FC$7$&  train-test&     $100$&  $99$&   $97$\\
GoogleNet&      pool5/7x7\_s1&  train-test&     $100$&  $99$&   $99$\\
VGG CNN S&      FC$7$&  train-test&     $100$&  $99$&   $99$\\
Places205 AlexNet&      FC$7$&  train-val&      $100$&  $99$&   $99$\\
Places205 Hybrid&       FC$7$&  train-val&      $100$&  $100$&  $100$\\
Flickr Style&   FC$8$ Flickr&   train-test&     $100$&  $100$&  $95$\\
Flickr Style&   FC$7$&  train-test&     $98$&   $41$&   $31$\\
\hline
CaffeNet&       FC$7$&  val-val&        $100$&  $98$&   $0$\\
\hline
            %
    %
    \end{tabular}}
                %
  \caption{Results for generating adversarials on various networks.  For each
      row, $100$ random samples are drawn from indicated splits of the dataset
      and optimized for $500$ iterations. {\it Out $\class{\source}$\/} is the
      number of adversarials that are predicted by the network to have
      a different label from source.  {\it In $\class{\guide}$\/} of the
      adversarials are predicted to be from the class of guide.
  $\guide=\neigh{1}{\adv}$ means the adversarial is so close to the guide that
  guide is its $1$NN\@.}
     %
 \label{tb:generalize_tb1}
%
\end{table*}

\begin{table*}[ht] \resizebox{\linewidth}{!}{\centering
        \begin{tabular}{|c|c|c|c|} \hline Model & Layer &Same $3$NN & Same
        $2/3$ 3NN\\ \hline
%
CaffeNet&       FC$7$&  $71$&   $24$\\
AlexNet&        FC$7$&  $72$&   $25$\\
GoogleNet&      pool5/7x7\_s1&  $87$&   $13$\\
VGG CNN S&      FC$7$&  $84$&   $16$\\
Places205 AlexNet&      FC$7$&  $91$&   $9$\\
Places205 Hybrid&       FC$7$&  $85$&   $15$\\
Flickr Style&   FC$8$ Flickr&   $100$&  $0$\\
Flickr Style&   FC$7$&  $28$&   $28$\\
\hline
CaffeNet&       FC$7$&  $70$&   $29$\\
AlexNet&        FC$7$&  $79$&   $20$\\
GoogleNet&      pool5/7x7\_s1&  $97$&   $3$\\
VGG CNN S&      FC$7$&  $79$&   $20$\\
Places205 AlexNet&      FC$7$&  $91$&   $9$\\
Places205 Hybrid&       FC$7$&  $84$&   $14$\\
Flickr Style&   FC$8$ Flickr&   $100$&  $0$\\
Flickr Style&   FC$7$&  $25$&   $30$\\
\hline
CaffeNet&       FC$7$&  $78$&   $20$\\
\hline
            %
    %
    \end{tabular}}
                %
  \caption{This table shows that for most of the time the nearest neighbors of
  the guide and the adversarial are exactly the same data points. The first
  column is the number of cases where all 3 nearest neighbors are the same.
  The second column is when 2 out of 3 are the same.}
     %
 \label{tb:generalize_tb1_2}
%
\end{table*}



\begin{table*}[ht] \resizebox{\linewidth}{!}{\centering
        \begin{tabular}{|c|c|c|c|c|c|c|} \hline Model Name & Layer & Split sets
        & Out $\class{\source}$& In $\class{\guide}$ & $\guide=\neigh{1}{\adv}$
        & $\rankdiff{3}$ median, [min, max]\\ \hline CaffeNet&       FC$7$&
        train-train&    $100$&  $95$&   $95$&   $-5.76, [-54.83, 0.00]$\\
        AlexNet&        FC$7$&  train-train&    $100$&  $97$&   $96$&   $-5.64,
        [-38.39, 0.00]$\\ GoogleNet&      pool5/7x7\_s1&  train-train& $100$&
        $100$&  $100$&  $-1.94, [-12.87, 0.10]$\\ VGG CNN S& FC$7$&
        train-train&    $100$&  $99$&   $99$&   $-3.37, [-26.34,
    0.00]$\\ Places205 AlexNet&      FC$7$&  train-train&    $100$&  $100$&
        $98$&   $-1.25, [-18.20, 8.04]$\\ Places205 Hybrid&       FC$7$&
        train-train&    $100$&  $99$&   $99$&   $-1.30, [-8.96, 8.29]$\\ Flickr
        Style&   FC$8$ Flickr&   train-train&    $100$&  $100$&  $95$&   $0.00,
        [0.00, 0.08]$\\ Flickr Style&   FC$7$&  train-train&    $98$&   $45$&
        $32$&   $-10.28,        [-37.35, -2.39]$\\ \hline CaffeNet&
        FC$7$&  train-test&     $100$&  $97$&   $96$&   $-5.37, [-27.38,
    0.00]$\\ AlexNet&        FC$7$&  train-test&     $100$&  $99$&   $97$&
        $-6.10, [-42.98, 0.23]$\\ GoogleNet&      pool5/7x7\_s1&  train-test&
        $100$&  $99$&   $99$&   $-1.62, [-10.18, 0.51]$\\ VGG CNN S&
        FC$7$&  train-test&     $100$&  $99$&   $99$&   $-3.36, [-18.21,
    0.73]$\\ Places205 AlexNet&      FC$7$&  train-val&      $100$&  $99$&
        $99$&   $-1.16, [-8.30, 3.25]$\\ Places205 Hybrid&       FC$7$&
        train-val&      $100$&  $100$&  $100$&  $-1.38, [-7.39, 5.87]$\\ Flickr
        Style&   FC$8$ Flickr&   train-test&     $100$&  $100$&  $95$&   $0.00,
        [0.00, 0.04]$\\ Flickr Style&   FC$7$&  train-test&     $98$&   $41$&
        $31$&   $-10.94,        [-28.96, 0.00]$\\ \hline CaffeNet&       FC$7$&
        val-val&        $100$&  $98$&   $-$&    $-6.29, [-25.58, -0.08]$\\
        \hline
            %
    %
    \end{tabular}}
                %
  \caption{Results for generating adversarials on various networks.  For each
      row, $100$ random samples are drawn from indicated splits of the dataset
      and optimized for $500$ iterations. {\it Out $\class{\source}$\/} is the
      number of adversarials that are predicted by the network to have
      a different label from source.  {\it In $\class{\guide}$\/} of the
      adversarials are predicted to be from the class of guide.
  $\guide=\neigh{1}{\adv}$ means the adversarial is so close to the guide that
  guide is its $1$NN\@.  Column of $\rankdiff{3}$ shows statistics for the
  difference of ranks.}
     %
 \label{tb:generalize_tb1_prev}
%
\end{table*}

\begin{table}[]
    \resizebox{\linewidth}{!}{\centering
        \begin{tabular}{|c|c|c|c|c|}
            \hline
            \multicolumn{5}{|c|}{train-train}\\
            \hline
Model name      &CaffeNet       &AlexNet        &GoogleNet      &VGG CNN S \\
\hline
CaffeNet &      100,95 &        61,3 &  42,0 &  53,1 \\
AlexNet &       61,0 &  100,97 &        46,0 &  57,0 \\
GoogleNet &     33,1 &  36,0 &  100,100 &       42,0 \\
VGG CNN S &     53,0 &  55,0 &  49,1 &  100,99 \\
            \hline
            \multicolumn{5}{|c|}{train-test}\\
            \hline
Model name      &CaffeNet       &AlexNet        &GoogleNet      &VGG CNN S \\
\hline
CaffeNet &      100,97 &        67,1 &  58,0 &  65,1 \\
AlexNet &       71,1 &  100,99 &        54,0 &  67,0 \\
GoogleNet &     50,0 &  49,1 &  100,99 &        48,0 \\
VGG CNN S &     59,2 &  57,0 &  61,0 &  100,99 \\
            \hline
        \end{tabular}
    }
\caption{Results for generating an adversarial for one network and testing it
on another network. The rows show the network for generating the adversarial
and the column shows the network used for testing the adversarials. For each
row, $100$ adversarials generated for Table~\ref{tb:generalize_tb1} is tested
on networks in the columns. Each cell shows the number of {\it Out
$\class{\source}$\/} and {\it In $\class{\guide}$}. } \label{tb:generalize_tb2}
%
\end{table}

}}}


==> exp_inv_fig_sara.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{\linewidth}
{
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{2pt}
\begin{tabular}{|
>{\centering\arraybackslash}m{0.15\linewidth}"
>{\centering\arraybackslash}m{0.15\linewidth}"
>{\centering\arraybackslash}m{0.15\linewidth}
>{\centering\arraybackslash}m{0.15\linewidth}
>{\centering\arraybackslash}m{0.15\linewidth}"
>{\centering\arraybackslash}m{0.15\linewidth}|}
\hline

Image & \vspace{0.2pt}$s_1$ & \vspace{0.2pt} $\alpha^{\text{FC}7}_{11}$ &\vspace{0.2pt}$\alpha^{\text{P}5}_{11}$ & \vspace{0.2pt}$\alpha^{\text{C}3}_{11}$ &\vspace{3pt} $g_1$  \\[1ex] \hline

Input & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730_43_conv3_t15/l10-orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/val_43.png} \\
Inv($\text{C}3$) & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l10-recon.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l10-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l10-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730_43_conv3_t15/l10-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l09-recon.png} 
\\
Inv($\text{P}5$) & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l15-recon.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730_43_conv3_t15/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l15-recon.png} 
\\
Inv($\text{FC}7$) & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l19-recon.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l19-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l19-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730_43_conv3_t15/l19-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l19-recon.png} 
\\

\hline
\end{tabular}
}
\end{subfigure}

\begin{subfigure}[t]{\linewidth}
{
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{2pt}
\begin{tabular}{|
>{\centering\arraybackslash}m{0.15\linewidth}"
>{\centering\arraybackslash}m{0.15\linewidth}"
>{\centering\arraybackslash}m{0.15\linewidth}
>{\centering\arraybackslash}m{0.15\linewidth}
>{\centering\arraybackslash}m{0.15\linewidth}"
>{\centering\arraybackslash}m{0.15\linewidth}|}
\hline
Image & 
\vspace{0.2pt}$s_2$ & \vspace{0.2pt} $\alpha^{\text{FC}7}_{22}$ & \vspace{0.2pt}$\alpha^{\text{P}5}_{22}$ &\vspace{0.2pt}$\alpha^{\text{C}3}_{22}$ &\vspace{3pt} $g_2$  \\[1ex] \hline

Input & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_27_conv3_t15/l10-orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27.png} \\
Inv($\text{C}3$) & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l10-recon.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l10-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l10-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_27_conv3_t15/l10-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l10-recon.png} 
\\
Inv($\text{P}5$) & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l15-recon.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_27_conv3_t15/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l15-recon.png} 
\\
Inv($\text{FC}7$) & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l19-recon.png} & 
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l19-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l19-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_27_conv3_t15/l19-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l19-recon.png} 
\\
\hline
\end{tabular}
}
\end{subfigure}
\caption{
In each of two panels, the top row shows a source image (left),
a guide image (right), and three adversarial images (middle) that were
optimized using layers FC$7$, P$5$, and C$3$ of caffenet.  The remaining three
rows show images reconstructed by inverting the DNN mapping from layers
C$3$, P$5$, and FC$7$.  From these images one can see how the internal
representation begins to mimic the guide, beginning with the layer
used for the optimization.  The representation was inverted using the
algorithm in~\cite{MahendranVedaldiCVPR2015}.
}
\label{fig:adv_invert}
\end{figure*}



\iffalse
\begin{figure*}[t!]
\centering
\renewcommand{\arraystretch}{0.3}
\setlength\tabcolsep{0pt}
\begin{tabular}{|>{\centering\arraybackslash}m{0.095\linewidth}"
>{\centering\arraybackslash}m{0.095\linewidth}>{\centering\arraybackslash}m{0.095\linewidth}
>{\centering\arraybackslash}m{0.095\linewidth}"
>{\centering\arraybackslash}m{0.095\linewidth}"
>{\centering\arraybackslash}m{0.095\linewidth}>{\centering\arraybackslash}m{0.095\linewidth}
>{\centering\arraybackslash}m{0.095\linewidth}"
>{\centering\arraybackslash}m{0.095\linewidth}|}
\hline

& & \vspace{0.2pt}$s_1$ & & \vspace{0.2pt} $g$& &\vspace{0.2pt} $s_2$ &  &\\[2ex] \hline
& \vspace{0.2pt} $\alpha^{\text{FC}7}_{11}$ &\vspace{0.2pt} $\alpha^{\text{P}5}_{11}$ &  \vspace{0.2pt}$\alpha^{\text{C}3}_{11}$ &\vspace{3pt} $g_1$  &\vspace{0.2pt} $\alpha^{\text{C}3}_{21}$ & \vspace{0.2pt}$\alpha^{\text{P}5}_{21}$  & \vspace{0.2pt}$\alpha^{\text{FC}7}_{21}$ & \vspace{5pt} $s_2$\\[1ex] \hline
Input &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_27mat/orig.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_27mat/orig.png} 
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730.png} 
 \\
\hline 
Inv($\text{C}3$) &
 \includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_27mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l09-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_27mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_27mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_27mat/l09-recon.png}
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l09-recon.png} 
\\
Inv($\text{P}5$) &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_27mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l15-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_27mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_27mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_27mat/l15-recon.png}
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l15-recon.png} 
\\
Inv($FC6$) &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_27mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l16-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_27mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_27mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_27mat/l16-recon.png}
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l16-recon.png} 
\\
Inv($\text{FC}7$) &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_27mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_27mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_27mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/27/l18-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_27mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_27mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_27mat/l18-recon.png}
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/730/l18-recon.png} 
\\
\hline
\vspace{5pt}$s_1$ & \vspace{0.2pt} $\alpha^{\text{FC}7}_{12}$ &\vspace{0.2pt} $\alpha^{\text{P}5}_{12}$ &  \vspace{0.2pt}$\alpha^{\text{C}3}_{12}$ &\vspace{3pt} $g_2$  &\vspace{0.2pt} $\alpha^{\text{C}3}_{22}$ & \vspace{0.2pt}$\alpha^{\text{P}5}_{22}$  & \vspace{0.2pt}$\alpha^{\text{FC}7}_{22}$ &\\[3ex] 
\hline
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie} 
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_100043mat/orig} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_100043mat/orig} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_100043mat/orig} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/val_43.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_100043mat/orig} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/orig} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/orig.png}
& Input
\\
\hline
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l09-recon.png} 
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_100043mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_100043mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_100043mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l09-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_100043mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l09-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l09-recon.png}
& Inv($\text{C}3$)
\\
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l15-recon} 
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_100043mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_100043mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_100043mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l15-recon} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_100043mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l15-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l15-recon.png}
& Inv($\text{P}5$)
\\
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l16-recon.png} 
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_100043mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_100043mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_100043mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l16-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_100043mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l16-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l16-recon.png}
& Inv($FC6$)
\\
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie/l18-recon.png} 
&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_fc7_100043mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t10_pool5_100043mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/pie_t20_conv3_100043mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/100043/l18-recon.png} &
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t20_conv3_100043mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_pool5_100043mat/l18-recon.png}&
\includegraphics[width=\linewidth,height=.75\linewidth]{./imgs/train_730_t10_fc7_100043mat/l18-recon.png}
& Inv($\text{FC}7$)
\\
\hline
\end{tabular}
\caption{In each of two panels, the top row shows a source image (left),
a guide image (right), and three adversarial images (middle) that were
optimized using layers FC$7$, P$5$, and C$3$ of caffenet.  The remaining three 
rows show images reconstructed by inverting the DNN mapping from layers 
C$3$, P$5$, and FC$7$.  From these images one can see how the internal 
representation begins to mimic the guide, beginning with the layer 
used for the optimization.  The representation was inverted using the 
algorithm in~\cite{MahendranVedaldiCVPR2015}. 
}
\label{fig:adv_invert}
\end{figure*}
\fi


==> exp_inv_sara.tex <==
\subsection{Inverting Internal Representations}

\input{exp_inv_fig_sara}

One way to examine the internal representations of the adversarial images,
as compared to the source and guide images, is to look at the images that 
they represent.  Do they look more like the source, the guide, or some
combination of the two?

Mahendran and Vedaldi \cite{MahendranVedaldiCVPR2015} formulate a 
way to invert the internal representation of any given layer of a DNN,
i.e., to invert the mapping $\phi_k^{-1}$.  
Beginning with random noise as an initial guess, they optimize
the following regularized objective using stochastic gradient descent
in order to find a reconstructed image $I_*$ with unit $L_2$ norm:
\begin{equation} 
\label{eq:inv_opt}
%
\frac{\lVert \Phi(\sigma I_*)-\Phi(I)\rVert^2_2 }{ \lVert \Phi(I) \rVert^2_2}
    +\lambda_\alpha\mathcal{R}_\alpha(I_*)+\lambda_{V^\beta}\mathcal{R}_{V^\beta}( I_* )
%
\end{equation}
where the two regularizers, $\mathcal{R}_\alpha(x)$ and 
$\mathcal{R}_{V^\beta}$, serve to produce natural images with a 
consistent dynamic range. Some form of regularization here is clearly
necessary because the DNN mapping is many-to-one.

The adversarial images generated by our optimization are designed to be 
close, if not perceptually equivalent, to a given source image (demonstrated 
in Fig.~\ref{fig:adv_caffenet}), with an internal represetation close to 
the guide. Fig.~\ref{fig:adv_invert} depicts reconstructed images for 
for two source images (chosen at random), each perturbed using two 
different guide images.  Since the quality of inverting convnet 
reconstructions is optimized for $100$ images in Imagenet validation 
set. the guides are chosen randomly from those in the validation set 
whose recunstruction was successful.

The results in Fig.~\ref{fig:adv_caffenet}) suggest that the internal 
representations of the adversarial images are indeed very close to those 
of the guide images.  The reconstructions do not appear similar to the 
sources images except for those done using layer C3, one of the lower 
conveolutional layers of caffenet.

\david{the conclusions here are somewhat weak ... can we sat more?}




==> exp_nnb_sara.tex <==
\subsubsection{Nearest Neighbor Distance Distribution
\fartash{Needs to be rewritten or removed}}
The manifold of natural image representations can be curved enough that it would not be well explained by a linear gaussian model anymore. Therefore, we further explore the extreme locality ($3$ nearest neighbors) of each point in this experiment.

We choose ImageNet training dataset as the sample of natural images and
calculate $\NNavg{3}{x}$ on FC$7$ representation of all of its images.
\iffalse Figure~\ref{fig:nnb_3_dist} suggests that the adversarials FC$7$
representations are inliers of the natural images FC$7$ representations. 
 Plots
in Figure~\ref{fig:nnb_3_dist}\subref{fig:nnb_imagenet} are distribution of
$\NNavg{3}{x}$ measure over ImageNet and validates normal distribution
assumption of $\NNavg{3}{x}$.\fi
The omnibus test of normality based on \cite{d1971omnibus} on the distribution of $\NNavg{3}{x} :x \in C_i$ shows that $89.8\%$ of the classes pass the null hypothesis with $p$-value greater than $0.05$. On average classes have $p$-value of $0.224$ which shows that there is no significant evidence that this distributions differ from a normal distribution.

Therefore, in order to verify whether an adversarial's $\NNavg{3}{\adv}$ is an inlier of its class
$\NNavg{3}{x}$ distribution we normalized $\NNavg{3}{\adv}$ by $\mu_i$ and $\sigma_i$ of its final class distribution $i$ and calculated the z-score of adversarial $\NNz{3}{x}$. Results show that on average adversarials are $0.15\sigma_i$ away from $\mu_i$ with standard deviation of $0.95$ which is less than $1$ $\sigma_i$ away from average of each class. More precisely, $88\%$ of adversarials are whithin $1$ standard deviation of their class distribution and less than $1\%$ are farther away than $2$ standard deviation.

These result, as a whole point to the fact that the adversarial images
are not far from natural images within the guide class, and cannot be
rejected out of hand as outliers.


\iffalse \begin{figure*}[t!]
\captionsetup[subfigure]{position=b}
\centering
%
\subcaptionbox{Histogram of $\NNavg{3}{x}$ for all $x$ in Imagenet training
dataset.  Left: distribution of all images in the dataset. Right: $3$ sample
distribution for all images within a class.\label{fig:nnb_imagenet}}
%
{\renewcommand{\arraystretch}{0} \setlength\tabcolsep{0pt} \centering
%
\begin{tabular}{@{}p{0.225\linewidth}p{0.225\linewidth}@{}}
%
    \includegraphics[width=\linewidth]{./imgs/each_3_nnb.png}
    & \includegraphics[width=\linewidth]{./imgs/each_3_samp.png}
%
\end{tabular}}
%
\subcaptionbox{Left: Histogram of $\NNz{3}{\adv}$.  Right: Plot of
$\NNz{3}{\adv}$ over the corresponding $\NNz{3}{\guide}$.  Left: The projection
of sorted values of right plot to the y-axis.
\label{fig:nnb_adv_dist}}
%
{\includegraphics[width=0.45\linewidth,
height=.2\linewidth]{./imgs/avg_3_nnb_10.png}}
%
\caption{Distributions of z-scores for average $3$-nearest neighbor distances,
$\NNz{3}{x}$.}\label{fig:nnb_3_dist} \end{figure*}

\fi


==> exp_understanding.tex <==
\subsection{TBD ``Understanding adv and causes"}

%\yanshuai{are intermediary rep out-of-subspace or in-subspace when upper rep is adv'ed}



==> fig_act_1.tex <==
\begin{figure*}[t!]
\centering
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{2pt}
\begin{tabular}{
>{\centering\arraybackslash}m{0.25\linewidth}
>{\centering\arraybackslash}m{0.25\linewidth}
>{\centering\arraybackslash}m{0.25\linewidth}
>{\centering\arraybackslash}m{0.25\linewidth}
}
1) Images & 2) Source & 3) Adversarial & 4) Guide \\
\begin{tabular}{
>{\centering\arraybackslash}m{0.45\linewidth}
>{\centering\arraybackslash}m{0.45\linewidth}}

\includegraphics[width=\linewidth, height=\linewidth]{./imgs/val_43.png} &
\includegraphics[width=\linewidth, height=\linewidth]{./imgs/ad_car_43.png} \\
\includegraphics[width=\linewidth, height=\linewidth]{./imgs/dif_car_43.png} &
\includegraphics[width=\linewidth, height=\linewidth]{./imgs/car.png} 
\end{tabular} &
\includegraphics[width=\linewidth]{./imgs/f7_43.png} &
\includegraphics[width=\linewidth]{./imgs/f7_car_43.png} &
\includegraphics[width=\linewidth]{./imgs/f7_car.png}
\end{tabular}
\caption{FC7 activation map of (Source, Adversarial, Guide) images in column 2, 
    3 and 4 respectively.  In the 1st column Source (top-left), $I_{\adv}^{\text{FC}7}$ 
      (top-right), guide(bottom-right) and difference of adversarial and source 
  (bottom-left) is depicted.}
\label{fig:act_f7}
\end{figure*}
\begin{figure*}[t!]
\centering
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{2pt}
\begin{tabular}{
>{\centering\arraybackslash}m{0.15\linewidth}
>{\centering\arraybackslash}m{0.28\linewidth}
>{\centering\arraybackslash}m{0.28\linewidth}
>{\centering\arraybackslash}m{0.28\linewidth}
}
1) Image & 2) Source & 3) Adversarial & 4) Guide \\
%\begin{tabular}{
%>{\centering\arraybackslash}m{\linewidth}}
\includegraphics[width=\linewidth, height=\linewidth]{./imgs/ad_car_43_p5.png} 
&
%\\
%\includegraphics[width=\linewidth, 
%height=\linewidth]{./imgs/dif_car_43_p5.png} \end{tabular} &
\includegraphics[width=\linewidth]{./imgs/p5_43.png} &
\includegraphics[width=\linewidth]{./imgs/p5_car_43.png} &
\includegraphics[width=\linewidth]{./imgs/p5_car.png}
\end{tabular}
\caption{Pool5 activation map of (Source, Adversarial, Guide) images in column 
2, 3 and 4 respectively.  In the 1st column $I_{\adv}^{\text{P}5}$ 
of the same (Source, 
Guide) as in Fig.~\ref{fig:act_f7} is depicted.
}
\end{figure*}


==> methodology.tex <==
% \subsection{Setup for Quantitative Analysis}

\iffalse
\input{sample_data}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{{{\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 Data Type & Imagenet Training & Imagenet Validation & Imagenet Test & Wikipedia & Total \\ \hline
Source\# & $5$ (R) & $5$ (R) + $3$ (M) & $5$ (R) & $3$ (M) & $20$ \\
Guide\# & $3300$ (PR) & $30$(PR) & $100$(R) & $0$ & $3430$ \\ \hline
\end{tabular}
}
\caption{Number of images from each data type present in each data set. 
R, PR and M stands for random, partially random and manual selection strategy.}
\label{data_table}
\end{table}
}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To this end we focus on the benchmark Caffenet, and random sets of 
source and guide images, some of which are shown in Fig.~\ref{data_figure}. 

\vspace*{0.05cm}
\noindent
{\em Source Set:} We report results on 20 source images.
Five were selected at random from the training, testing and validation 
sets of Imagenet.  Five more were selected manually from Wikipedia and 
the Imagenet validation set for greater diversity.

\vspace*{0.05cm}
\noindent
{\em GuildeL Set:} The large guide set is drawn from Imagenet data.  
This included three random images from each of the 1000 classes in the 
training set, along with 30 random images from the validation set -- 3030
images in total. To facilitate
quantitive analysis, we only selected those images whose labels are 
correctly predicted by caffenet.
\yanshuai{@Sara, What about the "30\_guides'' for training?}

\vspace*{0.05cm}
\noindent
{\em GuildeS Set:} This is subset of GuideL, comprising 3 random training 
images from each of 100 classes. It is used instead of GuideL solely for 
computational expedience. 

\vspace*{0.05cm}
\noindent
{\em GuideT Set:} We also consider a random set of 100 images from the 
Imagenet test set in order to explore whether test and training images 
produce advesarial images that are distinct in some way.  
\comment{
\begin{table}
\centering
\begin{tabular}{|m{0.45\linewidth}|m{0.15\linewidth}m{0.15\linewidth}m{0.15\linewidth}|}
    \hline
    Layer Name   & Pool 5 & FC 6 & FC 7 \\ \hline
    Dimension    & 9216 & 4096 & 4096 \\ \hline
    Mean of $avg_i$ & 1568.683    & 309.848    & 89.859   \\ \hline
    Maximum of $avg_i$ & 1904.253    & 418.522    & 115.334    \\ \hline
    Minimum of $avg_i$ & 1011.284    & 227.786    & 68.805    \\ \hline
    Average over all classes' maximum pairwise distance  & 2271.464    & 565.371    & 157.112    \\ \hline
\end{tabular}
\caption{Caffenet layer properties.
\david{Let's move the content of this table into the text in Section 4.2}}
\label{tab:caffenet}
\end{table}
}

In what follows, we generate an advesarial image from every combination
of source and guide images.  This yields 6660 pairs, in total, across the 
two disjoint guide sets.  
% The majority of our experimental results use the BVLC Caffe Refernce 
% model (caffenet).  A list of the layers of caffenet along with some 
% characteristics is given in Table~\ref{tab:caffenet}.  
All experiments on layer FC$7$ were done with GuideL (using all $1000$ 
classes).  For the remaining experiments we used GuideS (100 classes) 
for expedience.  Further experiments below 
% in  Sec.\ \ref{sec:exp_generalize} 
report results on other well-known convolutional neural networks. 




==> nn_analysis.tex <==
% \subsection{Nearest Neighbor Analysis}

\fartash{Why we can assume that euclidean distance in local neighborhoods is
meaningful?}

\comment{
%
If we assume that euclidean distance in local neighborhoods of a representation
is a meaningful measure of similarity, we can use non-parametric models to
compare our adversarial to the guide and other natural images. Given
a datapoint, the distance to its nearest neighbors (NNs) is related to the
density of datapoints in that local neighborhood.  For example, in high density
regions, datapoints are closer to each other and therefore the distance to top
nearest neighbors is smaller, and in low density regions, the nearest neighbors
are farther away.

Given that the computation of these measurements is fast, we also generalized
our analysis to other networks and show that we can generate adversarials on
networks other than Caffenet that are have CNN representations that are very
close to the guide and similar to natural images.

\subsubsection{Nearest Neighbor Measures}


\label{NNAnalysis}
Given the representation $x$ of a datapoint, let $\neigh{K}{x}$ be the $i$th
nearest neighbor of $x$ and $\Neighs{K}{x}$ the set of top $K$ nearest
neighbors of $x$. The average distance to $K$ top nearest neighbors is defined
as,

\begin{equation}
%
    \NNavg{K}{x} = \frac{\sum_{i=1}^{i=K} \dist{x}{\neigh{i}{x}}}{K}
\label{eq:3_nnb}
%
\end{equation}

We further use the z-score of $\NNavg{K}{x}$ defined as,
$\NNz{K}{x}=\frac{\NNavg{K}{x}-\mu}{\sigma}$, where. $\mu$ and $\sigma$ is
computed over the values of $\NNavg{K}{x} \forall x \in \class{\guide}$. An
adversarial that is close to its guide should be in the same region where the
value of $\NNz{K}{\adv}$ is very similar to $\NNz{K}{\guide}$ when compared to
other $\NNz{K}{x}$ for all other $x$ in that class.

Comparison of values of $\NNavg{K}{x}$ and $\NNz{K}{x}$, both depends on the
distribution of distances in a class. We define a rank measure $\rank{K}{x}$ to
remove this dependency. Let $\rank{K}{x}$ be the rank of $\NNavg{K}{x}$ in the
sorted order of all $\NNavg{K}{y} \forall y \in \class{\guide}$. Based on this
definition, the distribution of $\rank{K}{x}$ is uniform and therefore
comparable in different regions of space and in different representations. We
rescale the values of $\rank{K}{x}$ to be between $[0.0,
100.0]$, to represent percentiles.

We compare the rank of the adversarial to its guide by computing the difference
of their rank. Let $\rankdiff{K}(\adv,
\guide)=\rank{K}{\adv}-\rank{K}{\guide}$, be the difference. We expect
$\rankdiff{K}$ to be a small number when adversarials are close to the
$\guide$. 
%
}

